Use of a Socially Assistive Robot as a Online Shopping Digital Skills Assistan

This work proposes and analyses the application of a robotic platform as an digital skills assistant. analysing the ethical issues relating to the decision making process in the use case of online food shopping in order to inform a co design session on what, and how, the digital skills assistant should make decisions.

==> name.tex <==


\section{Tables}
\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

\section{Figures}

\begin{figure}[h]
  \centering
%  \includegraphics[width=\linewidth]{sampleteaser.pdf}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}
